Privacy-Preserving Identification of Target Patients from Outsourced Patient Data

With the increasing affordability and availability of patient data, hospitals tend to outsource their data to cloud service providers (CSPs) for the purpose of storage and analytics. However, the concern of data privacy significantly limits the data owners' choice. In this work, we propose the first solution, to the best of our knowledge, that allows a CSP to perform efficient identification of target patients (e.g., pre-processing for a genome-wide association study - GWAS) over multi-tenant encrypted phenotype data (owned by multiple hospitals or data owners). We first propose an encryption mechanism for phenotype data, where each data owner is allowed to encrypt its data with a unique secret key. Moreover, the ciphertext supports privacy-preserving search and, consequently, enables the selection of the target group of patients (e.g., case and control groups). In addition, we provide a per-query based authorization mechanism for a client to access and operate on the data stored at the CSP. Based on the identified patients, the proposed scheme can either (i) directly conduct GWAS (i.e., computation of statistics about genomic variants) at the CSP or (ii) provide the identified groups to the client to directly query the corresponding data owners and conduct GWAS using existing distributed solutions. We implement the proposed scheme and run experiments over a real-life genomic dataset to show its effectiveness. The result shows that the proposed solution is capable to efficiently identify the case/control groups in a privacy-preserving way.

==> 7_extra_operation.tex <==
\section{Discussion}
\label{sec:paper3_extension}
Here, we first discuss about the efficiency of the proposed scheme compared to purely fully homomorphic encryption (FHE)-based solutions. Then, we discuss how to extend our scheme to support other GWAS statistics. 
In Appendix \ref{sec:extension_proposed_scheme}, we also discuss the extensions of the proposed scheme for different applications.

\subsection{Efficiency Discussion}
Our scheme can be summarized in two phases.
The first phase is the identification of the case and control groups. 
The second phase is the computation of GWAS statistics (e.g., $\chi^2$ distribution test). 
As discussed, to the best of our knowledge, the proposed scheme is the first one to consider and provide privacy to both of these phases in a single framework. 
As we showed in Section~\ref{sec:paper3_evaluation}, the run-time for the first phase is more than 1000 times faster than the run-time of the second phase for a total number of 1052 patients (each having 263 SNPs) and 10 phenotypes in a query. As discussed, the performance of the second phase can be significantly improved via an optimized implementation of MKCKKS. 
As we also showed in Section~\ref{sec:paper3_evaluation_phenotype_search}, our proposed pairing-based encryption scheme is more than 20 times faster than FHE-based solutions for the first phase (in the second phase, we also propose using FHE for the calculation of statistics). 
Note that in many cases (e.g., optimal size of case and control groups or evaluate the similarity of patients), one needs to run the first phase more frequently than the second phase. 
%For instance, to find the optimal size of case and control groups or evaluate the similarity of patients, one may need to run the first phase several times (before executing or needing to run the second phase). 
Thus, the overall efficiency of the proposed scheme becomes significantly better than fully FHE-based solutions.


 \subsection{Calculating Other GWAS Statistics}
The proposed scheme can be easily extended to support calculating other GWAS statistics, e.g., p-value, minor allele frequency (MAF), and odds ratio. 
A p-value provides the probability showing whether a given result from a test is due to chance. Usually, if the p-value is less than 5 percent, it means the given result is highly due to the association, otherwise not.
%Since the $\chi^2$ distribution is a special case of the gamma distribution, 
%A  $\chi^2$ distribution with n degrees of freedom is equal to a gamma distribution with $a = n / 2$ and $b = 0.5 (or β = 2)$.
Based on the given result of $\chi^2$ distribution test (computed using Algorithm~\ref{alg:paper3_chi_square} in Section \ref{sec:paper3_computationovergenotypedata}), one can further obtain the p-value \cite{rana2015chi} by computing $p(x^2>v_{\chi^2)}$ where $v_{\chi^2}$  represents the  $\chi^2$ observation statistics and $x^2$ is the $\chi^2$ test statistics. 
Since the $\chi^2$ distribution is a special case of the gamma distribution, we can lookup the table and get the result (p-value). 
MAF provides information to differentiate between common and rare variants in a population. 
For a specific SNP, one can compute the MAF of a SNP as $\frac{\sum SNP.val}{2*(total~number~of ~individuals)}$, 
where numerator is the sum of the SNP values of all individuals and the denominator is two times of the total number of individuals. 
In our scheme, one can first homomorphically compute the numerator and denominator separately, and then compute the division homomorphically. 
For the odds ratio, the equation is $OR=\frac{D_E/N_E}{D_N/N_N}$, 
where $D_E$ is the number of individuals having a disease under certain condition (e.g., symptoms), $N_E$ is the total number of individuals (includes healthy people and patients) having the same condition,
$D_N$ is the number of individuals having a disease without the specific condition, and 
$N_N$ is the total number of individuals (include healthy people and patients) without the specific condition.  
%To further optimise the formula of odds ratio, 
%we can write $OR=\frac{D_EN_N}{D_NN_E}$.
First, the client can construct a query with disease and certain condition and send it to the CSP. Then, the CSP can compute $D_C$  without disclosing any information about the disease or certain conditions. 
Next, the client can construct a query only with the condition and obtains $N_E$. 
Similarly, the client can obtain $D_N$ and $N_N$. 
Finally, the odds ratio is computed without disclosing any information about disease or certain conditions of the individuals in the dataset. 





